Evaluation Cards: An Interpretive Layer for AI Evaluation Reporting

AI evaluation results are produced at scale but reported inconsistently across leaderboards, model cards, benchmark papers, and company blogs. The cost is interpretive: readers cannot reliably compare results across sources, identify what a report omits, or trace an aggregate claim to its underlying evidence. Recent efforts address isolated components but leave three gaps: they cover only narrow slices of the evaluation lifecycle and do not compose into a single interpretable record; they specify static representations that do not differentiate the questions different stakeholders bring to the same evidence; and they remain proposals on paper, lacking the extraction infrastructure required for adoption at scale. We present \EvalCards{}, an operational reporting layer that composes benchmark metadata, evaluation run data, and model metadata into a unified record. We (1) derive a reporting schema from a structured review of 52 papers and 10 stakeholder interviews, (2) implement four interpretive signals (reproducibility, documentation completeness, provenance and risk, and score comparability), rendered through reader modes calibrated to research and non-research audiences, and (3) deploy a monitoring tool that applies \EvalCards{} across 5,816 models, 635 benchmarks, and 101,843 results, surfacing systematic gaps in current reporting practice.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all claims in the abstract reflect the papers's scope and contributions. Contributions are then explained in detail in introduction. Applicable limitations are discussed in \Cref{app:limitations}. Where limitations form part of important analyses, these are discussed in the main body text.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Limitations are discussed in \Cref{app:limitations}. Where limitations form part of important analyses, these are discussed in the main body text.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No theoretical results are included in the paper.
    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The systematic review preregistration allows partial reproducibility of the included papers dataset, but certain search results, including the Google Scholar Results and Elicit are not stable and will not exactly reproduce. Similarly, expert inputs and interviews cannot be reproduced. The papers themselves are listed, and are publicly available.  The dataset of extracted items is available and can be verified or manually performed again, with correctness determined via the codebook. The extraction pipeline has open code that is reproducible, the data in the platform itself is available, and uploaded model evaluations themselves are (in-principle) reproducible depending on completeness of the provided data, continued availability of the models, and openness of the evaluations themselves. Limits to reproducibility of evaluations is a critical issue in the community, which is part of what is being addressed by the work presented in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do include an anonymized Github repository link to our code to reproduce, with the caveats outlined in the previous question, the main artifacts of the paper. Link: https://anonymous.4open.science/r/evalcards-anon-24EC/
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not run experiments requiring the specification of training and test details in this paper. We only compute the interpretative signals as outlined in \Cref{app:methodology}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % Error bars for inter-rater reliability are reported. 
    % Are there relevant places where the platform itself should do this / does or does not do so? (Perhaps the completeness signals, etc?)
    \item[] Justification: We report 95\% confidence intervals for inter-rater reliability statistics from the systematic review (\Cref{app:systematic-literature-review}). The four interpretive signals (reproducibility, completeness, provenance, comparability) are deterministic functions of the ingested corpus rather than estimates from repeated trials, so error bars are not applicable to their per-result computations; corpus-level rates (e.g., 96.5\% of triples flagged for reproducibility gaps) are descriptive summaries of the current corpus and we report exact counts and denominators alongside percentages throughout \Cref{app:walkthroughs}. We do not run evaluations ourselves and instead ingest first- and third-party results from existing sources, so reporting error bars on individual evaluation scores is out of scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve model training or evaluation runs. The EvalCards backend pipeline (ingestion, canonicalization, signal computation across 5,816 models, 638 benchmarks, and 101,955 results) runs on standard CPU infrastructure without GPU requirements (GitHub-hosted Linux runner, ubuntu-24.04 LTS, 4 vCPUs, 16 GiB RAM); a full corpus rebuild completes in under 20 minutes as of 6 May, 2026. The systematic literature review and interview coding were conducted manually and required no compute. We did not run preliminary experiments requiring substantial additional compute beyond what is reported. %\TODO{Add info about AutoBenchmarkCards compute use here --> Anka comment: I think this is fine for now to leave out given anonymity reasons & unclear if we actually need it because we only ingest it like EEE}  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conforms with the NeurIPS Code of Ethics. The interview component received IRB review (details withheld for anonymity). Participants gave informed consent prior to recording, were informed that quotes might be used and that they would be anonymized, and are reported under participant tags (P1-P5, T1-T5) without identifying details beyond role and region. The systematic literature review and corpus ingestion draw on publicly available sources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Evaluation Cards aim to improve the interpretability and accountability of public AI evaluation reporting by surfacing what is and is not documented for a given result, supporting more informed deployment, regulatory, and research decisions. By making reporting gaps visible across the corpus, it creates pressure toward more complete and reproducible evaluation practice without prescribing a particular reporting threshold. We see three concrete risks (discussed in \Cref{app:limitations}). First, safetywashing: developers may treat high completeness scores as evidence of evaluation quality when completeness measures only documentation adequacy, not the rigor of the underlying evaluation. We address this by stating the distinction explicitly in \Cref{sec:interprative-layer-signals} and by not assigning letter grades or pass/fail thresholds. Second, displacement: a unified reporting layer could crowd out alternative approaches to the same problem; we mitigate this through an open governance model (\Cref{app:governance}) that allows schema extensions and competing signal definitions. Third, normative entrenchment: the schema reflects choices about what counts as a complete evaluation, drawn from a literature that overrepresents English-language and frontier-scale work (\Cref{app:limitations}). Evaluation Cards inherit these biases, and surfacing them is a partial mitigation rather than a fix. The platform makes such assumptions visible to readers and contestable through the governance process, but cannot resolve them.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release pre-trained models, generative systems, or scraped datasets that pose dual-use or misuse risks. Evaluation Cards aggregates and structures publicly reported evaluation results from existing sources (Auto-BenchmarkCards, EEE, model metadata catalogs); no new model capabilities, training data, or sensitive content are introduced.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All existing assets used in the paper are cited with their original sources. The primary upstream data sources are Auto-BenchmarkCards (Apache 2.0 License), EEE (MIT License), hub-stats (Apache 2.0 License), and models.dev (MIT License), each cited at first use. The 52 papers in the systematic review are cited individually in \Cref{app:systematic-literature-review}. Software dependencies used in the canonicalization pipeline are open-source and used consistent with their licenses. %\TODO{Add specific licenses for ingested sources.}
    Evaluation Cards will be released under a CC-BY 4.0 license.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper introduces several new assets: (1) the \EvalCards{} reporting framework and schema; (2) the canonicalization pipeline and entity registry, with resolution accuracy validated on a sampled subset; and (3) the deployed monitoring platform and frontend. Documentation accompanies each asset: schema field specifications and population sources are in \Cref{app:evalcards-fields}, pipeline architecture and worked examples are in \Cref{app:data-normalization}, and limitations are stated in \Cref{app:limitations}. The systematic review materials are archived on OSF (link withheld for anonymity); all relevant code is anonymously released at \url{https://anonymous.4open.science/r/evalcards-anon-24EC/}. Regarding consent: \EvalCards{} aggregates publicly reported evaluation results from existing public sources. We did not seek individual consent from evaluation developers or model providers for inclusion of already-public information. Where evaluation developers contributed data directly to upstream sources (e.g., EEE), consent is governed by those sources' contribution policies. Verifying that upstream evaluations comply with the terms of service of the models they evaluate is the responsibility of the evaluators, not of \EvalCards{} as a downstream aggregator.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: 
    \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper involves human subjects in two ways. First, semi-structured interviews with 10 stakeholders informed the design and evaluation of \EvalCards{}. The full interview guide, recruitment approach, participant profile, and consent procedures are documented in \Cref{app:interview-methodology}. Participants were recruited through author networks and participated as part of their professional or research roles; no compensation was provided. Participants were informed prior to recording that interviews would inform an academic paper, that direct quotes might be used, and that all participants would be anonymized. Second, the systematic review involved expert feedback on screening decisions, codebook development, and framework synthesis from researchers active in AI evaluation; this feedback was provided as professional input within their existing roles and did not involve compensation. The corpus ingested by the Evaluation Card platform draws partially on community-contributed evaluation data via the EEE shared task \cite{evalevalcoalition2024}; instructions and compensation details for that task are documented in the cited reference.
    %The dataset used in the platform is partially crowdsourced. See discussion in \cite{evalevalcoalition2024} about the shared task.
    % DM Response: There were expert interviews and expert feedback on portions of the work, but because this is typically within the scope of their own employment or research responsibilities, did not involve compensation on our part.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The interview component received IRB review and was determined exempt prior to participant recruitment. The IRB details are withheld to preserve anonymity and will be provided in the camera-ready version. Risks to participants were minimal: interviews concerned professional perspectives on AI evaluation practice rather than sensitive personal information. Participants were informed before recording that the interview would inform an academic paper, that direct quotes might be used, and that all participants would be anonymized; consent was requested before any recording or AI note-taker use (\Cref{app:interview-methodology}). Participants are reported only by role tag (P1-P5, T1-T5), broad geographic region, and high-level role description, with no identifying details. The systematic literature review and corpus ingestion draw on publicly available materials and do not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLMs are used in this work in two methodologically relevant ways and several supporting roles. \textit{Methodologically relevant uses.} (1) Automatic categorization into the benchmark taxonomy used Claude Haiku 4-5. The first batch of LLM-generated categorizations was manually reviewed and corrected before the full run, and the resulting tags are stored as Evaluation Card annotations rather than written back to source records. (2) Auto-BenchmarkCards, one of \EvalCards{}' upstream sources, is itself LLM-generated; we ingest its output and inherit its validation guarantees and limitations. 
    \textit{Supporting uses (not affecting core methodology)}. Claude Sonnet 4.6 was used to generate Python code that transformed reviewer ratings from spreadsheet format and computed inter-rater agreement statistics; the underlying ratings and statistical procedures are reviewer-produced and standard. Claude was also used to generate initial cross-mappings between framework typologies during best-fit synthesis; all mappings were reviewed and revised by the authors before inclusion. LLM-based tools were used for diagram generation (LaTeX and TikZ figures) and for coding support on the platform frontend and backend (Claude Code with Opus 4.7).
    
    %Claude 4.6 used for generation of python code to transform reviewer ratings from original spreadsheet format and then calculate interrater statistics, as well as to generate the initial mappings between different typologies for the best-fit typology synthesis.\\
    %LLMs amd LLM-created tools were used for diagram generation and many of the Latex and Tikz diagrams used.\\
    %We used LLM to support coding in the platform front-end and back-end (Claude Code with Opus 4.7).

%For the methodology specified in Appendix~\ref{app:benchmark-taxonomy}, 
%Claude (claude.ai) was used for pipeline planning and phrasing. Anthropic API (claude-haiku-4-5) used for automatic categorization into taxonomy categories. The first batch of LLM-generated categorizations was manually reviewed and corrected before the full run proceeded.

    %%\justificationTODO{}

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> summary_tables.tex <==
\begin{table*}[t]
\centering
\caption{Quantitative summary spanning the corpus snapshot, model-level walkthrough (GPT-5), evaluation-level walkthrough (MMLU-Pro), and corpus-level interpretive signals.}
\label{tab:walkthrough-summary}
\scriptsize
\begin{tabular}{p{0.13\linewidth}p{0.23\linewidth}rrrp{0.27\linewidth}}
	\toprule
	Scope & Measure & $n$ & Denom.\ & Rate & Misc.\ \\
	\midrule
	Corpus snapshot & Models & $5{,}498$ & -- & -- & -- \\
	Corpus snapshot & Single benchmarks & $635$ & -- & -- & $62$ families \\
	Corpus snapshot & Reported results & $101{,}843$ & -- & -- & -- \\
	Corpus snapshot & Auto-BenchmarkCards & $211$ & -- & -- & $30$ organizations \\
	\addlinespace
	GPT-5 & Reported results & $213$ & -- & -- & $118$ benchmarks; $19$ organizations; $2$ source types \\
	GPT-5 & Missing reproducibility fields & $202$ & $213$ & $95.0\%$ & $11$ complete results \\
	GPT-5 & Benchmarks with Auto-BenchmarkCards & $64$ & $118$ & -- & $93.0\%$ completeness score \\
	GPT-5 & Benchmarks without Auto-BenchmarkCards & $54$ & $118$ & -- & $11.0\%$ completeness score \\
	GPT-5 & First-party results & $27$ & $213$ & $13.0\%$ & $186$ third-party or independent results ($87.0\%$) \\
	GPT-5 & MATH-500 score range & $3$ & -- & -- & $84.7\%$--$98.9\%$; $14.2$ point spread \\
	\addlinespace
	MMLU-Pro & Reported results & $5{,}079$ & -- & -- & $401$ models; $8$ organizations \\
	MMLU-Pro & Benchmark fields populated & $26$ & $28$ & $92.9\%$ & -- \\
	MMLU-Pro & Missing reproducibility fields & $4{,}975$ & $5{,}079$ & $98.0\%$ & $104$ complete results ($2.0\%$) \\
	MMLU-Pro & Third-party-only models & $383$ & $401$ & $95.5\%$ & $6$ first-party only; $12$ both \\
	MMLU-Pro & Multi-source models & $166$ & $401$ & $41.4\%$ & -- \\
	MMLU-Pro & Setup divergence cases & $11$ & -- & -- & $6$ cross-party divergence cases \\
	MMLU-Pro & Llama 3.2 score range & $2$ & -- & -- & $20.9\%$--$61.8\%$; $40.9$ point spread \\
	\addlinespace
	Corpus-level & Missing reproducibility triples & $48{,}698$ & $50{,}461$ & $96.5\%$ & $1{,}763$ complete triples ($3.5\%$) \\
	Corpus-level & max\_tokens missing & -- & -- & $95.6\%$ & temperature missing: $93.9\%$ \\
	Corpus-level & Agentic eval\_plan missing & -- & -- & $100.0\%$ & eval\_limits missing: $100.0\%$ \\
	Corpus-level & First-party field population & $180$ & -- & $0.0\%$ & Third-party field population on paired cases: $16.6\%$ \\
	Corpus-level & Median benchmark completeness & $635$ & -- & $10.7\%$ & Benchmarks with warehouse completeness rows \\
	Corpus-level & Single-party model--benchmark pairs & $48{,}968$ & $49{,}865$ & $98.2\%$ & $897$ multi-party pairs ($1.8\%$) \\
	Corpus-level & Divergent multi-party pairs & $65$ & $897$ & $7.2\%$ & $832$ non-divergent pairs ($92.8\%$) \\
	Corpus-level & Divergent metric groups & $94$ & $181$ & $51.9\%$ & -- \\
	Corpus-level & First-party-only prevalence & -- & -- & -- & $15.1\%$ agentic; $12.5\%$ general; $0.8\%$ safety \\
	\bottomrule
\end{tabular}
\end{table*}

